Sublinear Algorithms and Lower Bounds for Metric TSP Cost Estimation

We consider the problem of designing sublinear time algorithms for estimating the cost of a minimum metric traveling salesman (TSP) tour. Specifically, given access to a $n \times n$ distance matrix $D$ that specifies pairwise distances between $n$ points, the goal is to estimate the TSP cost by performing only sublinear (in the size of $D$) queries. For the closely related problem of estimating the weight of a metric minimum spanning tree (MST), it is known that for any $\varepsilon > 0$, there exists an $\tilde{O}(n/\varepsilon^{O(1)})$ time algorithm that returns a $(1 + \varepsilon)$-approximate estimate of the MST cost. This result immediately implies an $\tilde{O}(n/\varepsilon^{O(1)})$ time algorithm to estimate the TSP cost to within a $(2 + \varepsilon)$ factor for any $\varepsilon > 0$. However, no $o(n^2)$ time algorithms are known to approximate metric TSP to a factor that is strictly better than $2$. On the other hand, there were also no known barriers that rule out the existence of $(1 + \varepsilon)$-approximate estimation algorithms for metric TSP with $\tilde{O}(n)$ time for any fixed $\varepsilon > 0$. In this paper, we make progress on both algorithms and lower bounds for estimating metric TSP cost. We also show that the problem of estimating metric TSP cost is closely connected to the problem of estimating the size of a maximum matching in a graph.

==> app_lb.tex <==
\section{Omitted Details from Section~\ref{sec:ptas_lower_bound}} \label{sec:app-sat}
In this section, we give the formal proof of Theorem~\ref{thm:3SAT} and Theorem~\ref{thm:lb-TSP}.

\subsection{An $\Omega(n^2)$ Query Lower Bound for the $\Equ$ Problem}
We first prove a lower bound of $\Equ$ problem. $\Equ$ is the problem of deciding the satisfiability of a system of linear equations modulo 2, with three variables per equation.

We consider the following query model: the algorithm can query if an equation contains a variable. If the answer is \textbf{YES}, then the algorithm is also given all the variables and the right-hand side of the equation.

\begin{theorem} \label{thm:lbeq}
    For any $\eps>0$, any algorithm that distinguishes between a perfectly satisfiable $\Equ$ instance and an instance that satisfies at most $(1/2+\eps)$-fraction of equations needs $\Omega(n^2)$ queries with probability at least $2/3$.
\end{theorem}

We start by defining the hard distribution. The distribution is similar to the one in \cite{bogdanov2002lower}, but the query model and therefore the proof are different.
Every hard instance has $n$ variables $x_1,x_2,\dots x_n$ and $m=kn$ equations $e_1,e_2,\dots,e_m$ for some positive integer $k$. We construct the following two distributions of $\Equ$. 
\begin{itemize}
    \item The distribution $\dis_{NO}$ is the distribution of NO-instance, and is generated as follows: We first generate a random permuation $\sigma : [1,3m] \rightarrow [1,3m]$. For each $1\le i \le m$, we assign equation $e_i$ the variables $y^i_1=x_{\cei{\frac{\sigma(3i-2)}{3k}}}$, $y^i_2=x_{\cei{\frac{\sigma(3i-1)}{3k}}}$ and $y^i_3=x_{\cei{\frac{\sigma(3i)}{3k}}}$. The equation $e_i$ is $y^i_1+y^i_2+y^i_3 = \pm z_i$ where $z_i$ is choosen to be $+1$ or $-1$ uniformly randomly.
    \item The  distribution $\dis_{YES}$ is the distribution of YES-instance, and is generated as follows: We first assign the variables to each equation with the same process as $\dis_{NO}$. Then we randomly choose an assignment of vaiables, say $A^{\star}$. Finally, for each equation $e_i$, we set $y^i_1+y^i_2+y^i_3 = z_i$ where $z_i$ equals the sum of $y^i_1+y^i_2+y^i_3$ according to assignment $A^{\star}$.
\end{itemize}

Our final distribution generates an instance from the NO-distribution with probability $1/2$ and an instance from the YES-distribution with probability $1/2$.

If the instance is generated by $\dis_{YES}$, then it is satisfied by the assignment $A^{\star}$. The following lemma proves that if the instance is generated by $\dis_{NO}$, then with high probability, the at most $(1/2+\eps)$-fraction of the equations can be satisfied.

\begin{lemma} \label{lem:eqno}
    For any $\eps>0$, there exists a positive integer $k$, such that if an instance of $\Equ$ is randomly chosen from $\dis_{NO}$ with $n$ variables and $m = kn$ equations, then with probability $9/10$, at most $(1/2+\eps)$-fraction of the equations can be satisfied.
\end{lemma}

\begin{proof}
    Let $k = 8/\eps^2$ and so $m=\frac{8n}{\eps^2}$. Fix an assignment $A$. For each equation $e_i$, the probability that $A$ satisfies $e_i$ is $1/2$. Since in distribution $\dis_{NO}$, the right hand side of the equations are sampled independently, the event that $A$ satisfies any equation is independent of the event of $A$ satisfying any subset of the other equations. By the Chernoff bound, the probability that $A$ satisfies at least $(1/2+\eps)$-fraction of equations is at most $e^{-\frac{\eps^2 (m/2)}{4}} \le e^{-n}$. Taking the union bound over all possible assignments $A$, the probability that there exists an assignment that satisfies at least $(1/2+\eps)$-fraction of equations is at most $2^n \cdot e^{-n} < 1/10$.
\end{proof}

Now we prove that it is hard to distinguish between the YES and NO instances of this distributions. Define a bipartite graph $G_{\sigma}$  associated with the random permutation $\sigma$ as follows: there are $3m$ vertices on each side of $G_{\sigma}$, there is an edge between the $i^{th}$ vertex on the left and the $j^{th}$ vertex on the right if and only if $\sigma_i = j$. Since $\sigma$ is chosen uniformly at random, $G_{\sigma}$ is a randomly chosen perfect matching. Associate variable $x_i$ with the $(3k(i-1)+1)^{th}$ to the $(3ki)^{th}$ vertices on the left and associate equation $e_j$ with the $(3j-2)^{th}$ to the $(3j)^{th}$ vertex on the right. A variable occurs in an equation if and only if there is an edge between the vertices associate with the variable and the equation.

Fix an algorithm $\Alg$, let $\EE^{\Alg}_{YES}$ and $\EE^{\Alg}_{NO}$ be the set of equations given to $\Alg$ after all the queries to an instance generated by $\DYS$ and $\DNS$. Denote the knowledge graph $G^{\Alg}$ as the subgraph of $G_{\sigma}$ induced by the equations given to $\Alg$ and the variables that occur in these equations. The following lemma shows that if an algorithm only discover a small fraction of equations, then the set of equations discovered by the algorithm has the same distribution in the YES and NO cases with some high constant probability.

\begin{lemma} \label{lem:eqind}
    For any $k>0$, there exists a constant $\delta_0$ such that: if $G^{\Alg}$ contains at most $3 \delta_0 n$ edges, then the distributions of $\EE^{\Alg}_{YES}$ and $\EE^{\Alg}_{NO}$ are identical with probability at least $9/10$.
\end{lemma}

The proof of Lemma~\ref{lem:eqind} is similar to the proof of Theorem~8 in \cite{bogdanov2002lower}. We prove that the left hand side of the equations in $\EE^{\Alg}_{YES}$ and $\EE^{\Alg}_{NO}$ are independent, and thus the distribution of the right hand side are identical.

\begin{proof}
    We first prove that there is a constant $\delta_0$ such that with probability at least $9/10$, any set of equations of size $\delta n \le \delta_0 n$ contains more than $\frac{3}{2}\delta n$ variables. Fix a set of variables $V$ of size $\frac{3}{2}\delta n$. For any equation $e$, the probability that it contains only the variables in $V$ is $\frac{4.5 k \delta n}{3 k n} \cdot \frac{4.5 k\delta n-1}{3kn-1} \cdot \frac{4.5 k \delta n -2}{3kn-2} \le 4 \delta^3$. For any equation $e$ and any set of equations $\EE$ that does not contain $e$, the events that $e$ only contains variables in $V$ and the equations in $\EE$ only contain variable in $V$ are negatively correlated. So for any set of equations of size $\delta n$, the probability that these equations only contain variables in $V$ is at most $(4\delta^3)^{\delta n} = 4^{\delta n} \delta^{3\delta n}$. Taking the union bound over all possible set of equations of size $\delta n$, the probability that one of them only contains variables in $V$ is at most $4^{\delta n} \delta^{3\delta n} \cdot \binom{kn}{\delta n} \le 4^{\delta n} \delta^{3\delta n} \cdot (e k/\delta)^{\delta n} = (4ek)^{\delta n} \delta^{2\delta n}$. We now take the union bound over all sets of variables of size $\frac{3}{2}\delta n$; the probability that there exists a set of equations of size $\delta n$ which only contains $\frac{3}{2}\delta n$ variables is at most $(4ek)^{\delta n} \delta^{2\delta n} \cdot \binom{n}{1.5 \delta n} \le (4ek)^{\delta n} \delta^{2\delta n} \cdot (\frac{2e}{3\delta})^{1.5\delta n} \le (3e^{2.5}k)^{\delta n} \delta^{0.5\delta n} = (40k \sqrt{\delta})^{\delta n} \le (40k \sqrt{\delta_0})^{\delta n}$. Let $\delta_0 < \frac{1}{11 (40k)^2}$, and taking union bound over all possible sizes $i$ ranging from $1$ to $\delta_0 n$, the probability that any set of equations of size $i \le \delta_0 n$ contains more than $\frac{3}{2} i$ variables is at least $1 - \sum_{i=1}^{\delta_0 n} (\frac{1}{11})^i \ge 9/10$. 

    So with probability at least $9/10$, any set of equations with size $i \le \delta_0 n$ contains more than $\frac{3}{2}i$ variables, which means there is at least one variable that occurs at most once in these equations by the pigeonhole principle. We prove that under this event, the distribution of $\EE^{\Alg}_{YES}$ and $\EE^{\Alg}_{NO}$ are identical if $G^{\Alg}$ contains at most $3 \delta_0 n$ edges. 

    Notice that the left hand side of of $\EE^{\Alg}_{YES}$ and $\EE^{\Alg}_{NO}$ are always identical, we only need to prove that the distributions of the right hand side are identical when $G^{\Alg}$ has at most $3 \delta_0 n$ edges. In this case there are at most $\delta_0 n$ equations in $\EE^{\Alg}_{YES}$ since each equation is associated with 3 vertices. Let the right hand sides of $\EE^{\Alg}_{YES}$ and $\EE^{\Alg}_{NO}$ be vectors $b_{YES}$ and $b_{NO}$ respectively. We prove the distributions of $b_{YES}$ and $b_{NO}$ are identical by induction on the size of $b_{YES}$ (which is also the number of equations in $\EE^{\Alg}_{YES}$). 

    The base case is when there is no equation in $\EE^{\Alg}_{YES}$ at all (which means the algorithm does not discover any equation). In this case, both $b_{YES}$ and $b_{NO}$ are empty vectors.

    In the induction step, $\card{b_{YES}} = \card{b_{NO}} > 0$. Since the number of equations is at most $\delta_0 n$, there exists a variable $v$ that only occurs once. Without loss of generality, suppose it occurs in the last equation. Let $b'_{YES}$ and $b'_{NO}$ be the vector obtained by deleting the last entry of $b_{YES}$ and $b_{NO}$ respectively. By induction hypothesis, the distributions of $b'_{YES}$ and $b'_{NO}$ are identical. Moreover, $v$ only occurs in the last equation and only occurs once, the distribution of the last entry of $b_{YES}$ is uniform, independent of the other entries, so is the last entry of $d_{NO}$. So the distributions of $b_{YES}$ and $b_{NO}$ are identical.
\end{proof}

Next we prove that in order to discover a constant fraction of equations, we need $\Omega(n^2)$ queries.

\begin{lemma} \label{lem:eqquery} 
    For any $\delta_0>0$, there exists a $\delta_1>0$ such that: for any algorithm that makes at most $\delta_1 n^2$ queries, $G^{\Alg}$ contains at most $3 \delta_0 n$ edges with probability $9/10$.
\end{lemma}

The proof of Lemma~\ref{lem:eqquery} is similar to the proof of Theorem~5.2 in \cite{assadi2019sublinear} and we will prove it later.

\begin{proof}[Proof of Theorem~\ref{thm:lbeq}]
    For any $\eps>0$, let $k,\delta_0,\delta_1$ be the constant defined in Lemma~\ref{lem:eqno}, Lemma~\ref{lem:eqind}, Lemma~\ref{lem:eqquery} respectively. Consider two instance $I_{YES}$ and $I_{NO}$ generated as follows: we generate the instance $I_{YES}$ by distribution $\dis_{YES}$, then let the left hand side of $I_{NO}$ be the same as the left hand side of $I_{YES}$, generate the right hand side of $I_{NO}$ uniformly independently for each equation. Since the process of generating the left hand side is the same for $\dis_{YES}$ and $\dis_{NO}$, the distribution of $I_{NO}$ is indeed $\dis_{NO}$. By Lemma~\ref{lem:eqno}, with probability $9/10$, the $I_{NO}$ satisfies at most $(1/2+\eps)$-fraction of equations. By Lemma~\ref{lem:eqquery}, if an algorithm makes at most $\delta_1 n^2$ queries, then it discovers at most $\delta_0 n$ equations with probability $9/10$. Base on this event, by Lemma~\ref{lem:eqind}, the equations discovered by the algorithm has the same probability of being generated by $\dis_{YES}$ and  by $\dis_{NO}$. By the union bound, with probability at most $7/10$, $I_{NO}$ is an instance that satisfies at most $(1/2+\eps)$-fraction of the equations and the algorithm cannot distinguish between $I_{YES}$ and $I_{NO}$.
\end{proof}

\input{app_lower_bound}


\subsection{Reduction from $\Equ$ to 3SAT}

We use the following standard reduction from Equation to 3SAT in \cite{haastad2001some}.
Given a set of equations $\EE$, we construct a 3CNF formula $\Phi = F(\EE)$ as follows: For any equation $X_i+X_j+X_k=1$ in $\EE$, we add four clauses $(X_i \vee X_j \vee X_k)$, $(X_i \vee \bar{X_j} \vee \bar{X_k})$, $(\bar{X_i} \vee X_j \vee \bar{X_k})$ and $(\bar{X_i} \vee \bar{X_j} \vee X_k)$ into $\Phi$; for any equation $X_i+X_j+X_k=0$ in $\EE$, we add four clauses $(\bar{X_i} \vee X_j \vee X_k)$, $(X_i \vee \bar{X_j} \vee X_k)$, $(X_i \vee X_j \vee \bar{X_k})$ and $(\bar{X_i} \vee \bar{X_j} \vee \bar{X_k})$ into $\Phi$. It is clear that if an assigment satisfies an equation in $\EE$, then it also satisfies all of the four corresponding clauses in $\Phi$. Otherwise it satisfies three of the four corresponding clauses. So we have the following lemma.

\begin{lemma}  \label{lem:red-eq-3sat}
    For any $\gamma \in (0,1]$, given a set of equations $\EE$ and its corresponding 3CNF formula $\Phi = F(\EE)$, for any assignment $A$, $A$ satisfies $\gamma$-fraction of equations in $\EE$ if and only if $A$ satisfies $(3/4+\gamma/4)$-fraction of clauses in $\Phi$.
\end{lemma}

\begin{proof} [Proof of Theorem~\ref{thm:3SAT}]
    For any 3CNF formula generated from a $\Equ$ instance $\EE$ we consider a stronger type of query model for 3SAT. For any query between a variable and a clause, if the variable occurs in the clause, then the algorithm is not only given the entire clause, but also the other 3 clauses corresponding to the same equation in $\EE$. The new query is equivalent to the query in $\Equ$.
\end{proof}

\iffalse
\subsection{Proof of Theorem~\ref{thm:lb-TSP}}
\begin{theorem*} [Restatement of Theorem~\ref{thm:lb-TSP}]
  There is a constant $\eps_0$ such that any algorithm that approximates the $(1,2)$-TSP cost to within a factor of $(1+\eps_0)$ needs $\Omega(n^2)$ queries.
\end{theorem*}

We consider the following stronger queries for $(1,2)$-TSP: for any query $(u,v)$, if $u$ is in a vertex gadget $G_{x_j}$ and $v$ is in a clause gadget $G_{c_i}$ (or vice versa) and $x_j$ occurs in $c_i$ in the 3SAT instance, then the algorithm is given all the edges incident on $G_{c_i}$. Otherwise the algorithm just learns if the there is an edge between $u$ and $v$.

Let $\eps = 1/16$, and let the values of $k$, $L$ and $N$ correspond to this choice for $\eps$ according to the redution in Section~\ref{sec:lb-TSP}. Let $\eps_0 = \frac{k}{32(k+3)L}$. Consider the $(1,2)$-TSP instance reduced from the 3SAT instance generated by the hard distribution in Theorem~\ref{thm:3SAT} with $\eps = 1/16$. If the 3SAT instance is perfectly satisfiable, then the $(1,2)$-TSP instance has a Hamilton cycle of cost $N$. If the 3SAT instance satisfies at most $(15/16)$-fraction of clauses, then each Hamilton cycle in the $(1,2)$-TSP instance has cost at least 
$$N+(1/8-\eps)m/2 = N+(1/8-\eps)kn/6 \ge (1+\frac{(1/8-\eps)k}{2(k+3)L})N = (1+\eps_0) N$$

For any query $(u,v)$ in the $(1,2)$-TSP instance, we can simulate it by at most one query in the corresponding 3SAT instance as follows: if $u$ is in a vertex gadget $G_{x_j}$ and $v$ is in a clause gadget $G_{c_i}$ (or vice versa), then we make a query of $x_j$ and $c_i$ in the 3SAT instance. If the 3SAT query returns YES and the full information of $c_i$, then we return all the edges incident on $G_{c_i}$ according to the reduction rule and the full information of $c_i$. If the 3SAT query returns NO or $(u,v)$ are not in a vertex gadget and a clause gadget respectively, we return YES if $(u,v)$ is an edge in the ground graph and NO otherwise.

By Theorem~\ref{thm:3SAT}, any algorithm that distinguishes a perfectly satisfiable 3SAT instance from an instance where at most $(15/16)$-fraction of the clauses can be satisfied needs $\Omega(n^2)$ queries. So any algorithm that distinguishes a $(1,2)$-TSP instance containing a Hamilton cycle of length $N$ from an instance that has minimum Hamilton cycle of cost $(1+\eps_0)N$ needs $\Omega(n^2)$ queries.
\fi

==> app_one_two.tex <==
\section{Proof of Lemma~\ref{lem:mat-pair}} \label{sec:app-ot}
The algorithm that approximates the size of a maximal matching pair is almost the same as the algorithm that approximates the size of a maximal matching in \cite{onak2012near}, which is built on the algorithm that approximates the size of a maximal independent set in \cite{yoshida2012improved}. 



The algorithm in  \cite{onak2012near} constructs a maximal matching $M$ in a given graph $G$ as follows. We generate a random rank function $\pi$ on the edges of $G$, (which imposes a random permutation order on the edges,) and consider the edges one by one from lower rank to higher rank. When considering $e$, if there is no edge $e'$ in $M$ in conflict with $e$, then we add $e$ into $M$. 

Given the ranking $\pi$, the oracle $MO^{\pi}(e)$ (Algorithm~\ref{alg:O_M}) checks if the edge $e \in G$ is in $M$. The oracle $VO^{\pi}(v)$ (Algorithm~\ref{alg:O_V}) checks if a vertex $v \in G$ is matched in $M$. 



\begin{algorithm}[h] 
Let $e_1,\ldots,e_t$ be the edges incident to the vertex $v$ in order of increasing rank. \;
\For {$i=1,\ldots, t$}{ 
    \If { $MO^{\pi}(e_i) =$~{\sc true}}{ \Return {\sc true}} 
    \Return {\sc false} 
}
\caption{$VO^{\pi}(v)$: Check if a vertex $v$ is matched \cite{onak2012near}} \label{alg:O_V}
\end{algorithm}

\begin{algorithm}[h] 
\If {$MO^{\pi}(e)$ has already been computed}{\Return the computed answer.}
Let $e_1,\ldots,e_t$ be the edges that conflict with $e$, in order of increasing rank.\;
$i \leftarrow 1$.\;
\While {$\pi(e_i) < \pi(e)$}{
    \If {$MO^{\pi}(e_i) =$~{\sc true}}{\Return {\sc false}} 
    $i \leftarrow i+1$.
} \Return {\sc true} 
\caption{ $MO^{\pi}(e)$: Check if an edge $e$ is in the matching \cite{onak2012near}} \label{alg:O_M}
\end{algorithm}

The algorithm will sample $O(1/\eps^2)$ vertices in $G$ and call $VO^{\pi}$ on each one to check if it is matched in $M$. By Chernoff bound, we have an approximation of the size of $M$ with additive error $O(\eps n)$. 

Let $d_{\max}$, $d_{\min}$ and $\bar{d}$ be the maximum degree, minimum degree and average degree of $G$ respectively. The following two lemmas are proved in \cite{onak2012near}. We will later modify the statement of these lemmas and their proofs in order  to apply them to the maximal matching pair problem. 

\begin{lemma}\cite{onak2012near} \label{lem:old-ot-main}
For any graph $G$ (that may contains parallel edges and self loops), if we randomly choose a permutation $\pi$ and a vertex $v$ in $G$, the expected number of calls to $MO^{\pi}$  when we call $VO^{\pi} (v)$ is $O(\frac{d_{\max}}{d_{\min}} \cdot \bar{d})$.
\end{lemma}

Lemma~\ref{lem:ot-main} only gives an upper bound on the number of calls of $MO^{\pi}$, not on the number of queries needed. We may need to query all edges incident on a vertex to figure out which  $MO^{\pi}$ calls to make. Fortunately, \cite{onak2012near} (see Section~4 in \cite{onak2012near} for details) gives a technique for ``permutation generation on the fly'' which helps upper bound the number of queries made when calling $VO^{\pi}$ on a random vertex $v$ in $G$ in the neighbor query model. This technique will also be used in the proof of our modified lemmas.

\begin{lemma}\cite{onak2012near}  \label{lem:old-ot-nei}
For any graph $G$ (that may contains parallel edges and self loops), if we randomly choose a permutation $\pi$ and a vertex $v$ in $G$, then the expected number of neighbor queries used when calling $VO^{\pi}$ is $\tilde{O}(\frac{d_{\max}}{d_{\min}} \cdot \bar{d})$.
\end{lemma}


There are 3 challenges in extending the ideas in \cite{onak2012near} to our problem; the first two of these are already handled in \cite{onak2012near}. 1) We need to simulate the algorithm using neighbor queries by an algorithm that uses pair queries. 2) We need to bound the ratio $d_{\max} / d_{\min}$ in Lemma~\ref{lem:ot-nei}. 3) We need to extend their lemmas from generating one maximal matching to generating a maximal matching pair. To achieve the first two goals, we follow \cite{onak2012near} to construct a new graph $G'$ such that the maximal matching pair in $G'$ is close to the maximal matching pair in $G$. 


Suppose the vertex set of $G$ is $\{v_1,v_2,\dots,v_n\}$. The graph $G'$ has $2$ sets of vertices $V^1_{G'}$ and $V^2_{G'}$, where $V^1_{G'} = \{v^1_1,\dots,v^1_n\}$ and $V^2_{G'} = \{v^2_1,\dots,v^2_n\}$. For any $i$, $v^1_i$ has degree $n$ and $v^2_i$ has degree $\frac{32n}{\eps}+n$. For any $j \le n$, if $(v_i,v_j)$ is an edge in $G$, then the $j^{th}$ neighbor of $v^1_i$ is $v^1_j$ and the $j^{th}$ neighbor of $v^2_i$ is itself. If $(v_i,v_j)$ is not an edge in $G$, then the $j^{th}$ neighbor of $v^1_i$ is $v^2_i$ and the $j^{th}$ neighbor of $v^2_i$ is $v^1_i$. For any $n < j \le 32n/\eps+n$, the $j^{th}$ neighbor of $v^2_i$ is itself. By construction of $G'$, any neighbor query on $G'$ can be simulated by at most 1 pair query on $G$. Note that since $G$ does not have self-loops,
the only self-loops in $G'$ are on vertices in $V^2_{G'}$. It is also clear that the ratio of the maximum and minimum degrees in $G'$ is $O(\frac{1}{\eps})$.

To achieve the third goal, we further modify $G'$ and construct a graph denoted $H$ consisting of two copies of $G'$.   So a vertex $v^{\ell}_i$ in $G'$ for $\ell \in \{1,2\}$ and $i \in [1,n]$ becomes two vertices, $u^{\ell}_i$ and $w^{\ell}_i$ in $H$. For any self loop on vertex $v^2_i$ in $G'$, we replace the two self loops in $H$, by an edge between $u^2_i$ and $w^2_i$. As before, two edges in $H$ conflict if they share an endpoint. In addition, an edge that arises from a non-self-loop edge in $G'$ conflicts with its duplicate in $H$. See Figure~\ref{fig:one-two} as an illustration. Note that in this construction, $H$ has no self loops. 

\input{fig-one-two}

We now state  the modifications of Lemmas \ref{lem:old-ot-main} and \ref{lem:old-ot-nei} with the new definition of conflict in $H$. We will also provide the proof of Lemma \ref{lem:ot-main} in Section~\ref{sec:ot-main}. The proof of
Lemma \ref{lem:ot-nei} follows along the same lines as the proof in \cite{onak2012near}.

\begin{lemma}\label{lem:ot-main}
Let $H$ be any graph constructed from a graph $G$ that does not contain self-loops,  using the two-step process above.  If we randomly choose a permutation $\pi$ and a vertex $v$ in $H$, the expected number of calls to $MO^{\pi}$  when we call $VO^{\pi} (v)$ is $O(\frac{n}{\eps^2})$.
\end{lemma}

\begin{lemma} \label{lem:ot-nei}
For $H$ as above, if we randomly choose a permutation $\pi$ and a vertex $v$ in $H$, then the expected number of neighbor queries used when calling $VO^{\pi}$ is $\tilde{O}(\frac{n}{\eps^2})$.
\end{lemma}

\begin{proof} [Proof of Lemma~\ref{lem:mat-pair}]

Let $V^1_H$ and $V^2_H$ be the set of vertices in $H$ which corresponding to the vertices in $V^1_{G'}$ and $V^2_{G'}$ respectively. Note that $|V^1_H| = |V^2_H| = 2n$. The algorithm works as follows: we sample $N = 100 /\eps^2$ vertices in $V^1_H$, and call $VO^{\pi}$ on them. Suppose $\bar{Y}$ is the number of times that $VO^{\pi}$ returns {\sc true}. Output $\frac{\bar{Y}n}{N}$ as our estimate of the size of the matching pair in $G$.

We first bound the number of pair queries used in this algorithm. By Lemma~\ref{lem:ot-nei}, if we randomly choose a vertex $v$ in $H$, the expected number pair queries $G$ used when calling $VO^{\pi}(v)$ is $ \tilde{O}(n/\eps^2)$. On the other hand, since $V^1_H$ contains half of the vertices in $H$, if we choose $v$ randomly inside $V^1_H$, the expected number of pair queries used when calling $MO^{\pi}(v)$ is also $\tilde{O}(n/\eps^2)$. By Markov's inequality, the algorithm uses $\tilde{O}(n/\eps^4)$ pair queries with probability at least $9/10$. 

Let $M^{\pi}$ be the set of edges in $H$ such that $MO^{\pi}$ returns {\sc true}. Note that $M^{\pi}$ is a matching  in $H$. Let $Y$ be the number of vertices in $V^1_H$ that are matched in $M^{\pi}$. By Chernoff bound $\card{\frac{2 \bar{Y} n}{N} - Y} \le \eps n/2$ with probability at least $9/10$.

We are interested only in the matching induced on $V^1_H$ because this corresponds to a matching pair in $G$. In order to show that the matching we find will mostly match vertices in $V^1_H$ to vertices in
$V^1_H$, we prove that if we choose permutation $\pi$ randomly, there are only a few vertices in $V^{H}_1$ are matched to vertices in $V^{H}_2$.  The only edges between $V^1_H$ and $V^2_H$ are between $u^1_i$ and $u^2_i$ or between $w^1_i$ and $w^2_i$ and we want to show that these edges are not used much in the matching. For any index $i$, if among all the edges incident on $u^2_i$ and $w^2_i$, the lowest rank edge is between $u^2_i$ and $w^2_i$, then $u^2_i$ and $w^2_i$ are matched to each other in $M^{\pi}$, and thus $u^1_i$ and $w^1_i$ are not matched to a vertex in $V^2_H$. By construction of $G'$, $v^2_i$ has at least $32n/\eps$ self loops, so there are at least $32n/\eps$ parallel edges between $u^2_i$ and $w^2_i$ in $H$. On the other hand, there are at most $n$ edges incident on $v^2_i$ that are not self loops, so there are at most $32n/\eps + 2n$ edges incident on $u^2_i$ and $w^2_i$. With probability at least $1- \eps/16$, $u^2_i$ is matched to $w^2_i$. Let $S$ be the set of indices $i$ such that $u^2_i$ is matched to $w^2_i$ in $M^{\pi}$. By Chernoff bound, $\card{S} \ge n - \eps n/8$ with probability at least $9/10$.

Let $U_S$ be the set of $u^1_i$ such that $i \in S$ and $W_S$ be the set of $w^1_i$ such that $i \in S$. Let $M'_1$ be the set of edges in $M^{\pi}$ that are incident on $U_S$ and $M'_2$ be the set of edges in $M^{\pi}$ that are incident on $W_S$. Let $M_1$ and $M_2$ be the set of edges in $G$ that correspond to the edges in $M'_1$ and $M'_2$ respectively. By definition of $MO^{\pi}$, $M_1$ and $M_2$ are both matchings in $G$ and $M_1 \cap M_2 = \emptyset$. Let $V_S$ be the set of vertices $v_i$ such that $i \in S$ and $G_S$ be the subgraph of $G$ induced by $V_S$. For any edge $(v_i,v_j)$ in $G_S$ that is not in $M_1 \cup M_2$, either $u^1_i$ or $u^1_j$ is matched in $M'_1$ and either $w^1_i$ or $w^1_j$ is matched in $M'_2$. So $(M_1,M_2)$ is a maximal matching pair in $G_S$. Suppose $X$ is the size of $(M_1,M_2)$. Let $(M_1^{\star},M_2^{\star})$ be an arbitrary maximal matching pair in $G$ such that $M_1 \subseteq M^{\star}_1$ and $M_2 \subseteq M^{\star}_2$. $(M^{\star}_1,M^{\star}_2)$ has size $X^{\star} \le X + 2(n-\card{S}) = X + \eps n / 4$.

On the other hand, by definition of $X$, there are $2X$ vertices in $U_S$ and $W_S$ that are matched in $M^{\pi}$, and we have $\card{V^1_H \setminus (U_S \cup W_S)} \le 2(n-s) \le \eps n / 4$. So $Y \ge 2X \ge Y-\eps n / 4$. So $\card{X^{\star}-\frac{\bar{Y}n}{N}} \le \eps n /4 + \eps n /4 + \eps n/8 < \eps n$. The failure probability is at most $1/10+1/10+1/10 < 1/3$ by union bound.
\end{proof}


\subsection{Proof of Lemma~\ref{lem:ot-main}} \label{sec:ot-main}

In this section, we focus on the graph $H$ and hence we redefine our notation. Let $H=(V,E)$ and let $n=\card{V}$ and $m=\card{E}$. (Note that in the notation of the previous proof, the number of vertices in $H$ would actually have been $4n$.)  We also adopt some notation from \cite{onak2012near}. Let $\Pi$ be the set of all possible permutations. Given a permutation $\pi$ and a vertex $v \in H$, $N(\pi,v)$ is the number of calls of $MO^{\pi}$ when calling $VO^{\pi}(v)$. Since the maximum degree of $H$ is $32n/\eps + n$ and the minimum degree of $H$ is $n$, to prove Lemma~\ref{lem:ot-main}, it is sufficient to prove 
$$
\frac{1}{n} \cdot \frac{1}{m!} \cdot \sum_{\pi \in \Pi} \sum_{v \in V} N(\pi,v) = O\Paren{\frac{d_{\max}}{d_{\min}} \cdot \bar{d}}
$$

For any edge in $H$, we arbitrarily denote $v_a(e)$ and $v_b(e)$ to be the endpoints of $e$. For a ranking $\pi$ and an index $k$, let $\pi_k$ be the edge $e$ such that $\pi(e)=k$. If two edges $e$ and $e'$ share only one endpoint, denote $v_c(e,e')$ as the common endpoint, and $v_d(e,e')$ as the endpoint of $e$ that is not an endpoint of $e'$.

For an edge $e$ and a vertex $v$, let $X^{\pi}(v,e)=1$ if $MO^{\pi}$ is called when calling $VO^{\pi}(v)$, and $X^{\pi}(v,e)=0$ otherwise. By definition of $MO^{\pi}$ and $VO^{\pi}$, we have
    $$
N(\pi,v) = \sum_{e \in E} X^{\pi}(v,e)
    $$
    Also, for any edge $e\in E$ and index $k$, define $X_k(e)$ to be
    $$
    X_k(e)=\sum_{\pi \in \Pi} \Paren{X^{\pi}(v_a(\pi_k),e)+X^{\pi}(v_b(\pi_k),e) }
    $$
    By definition of $X_k(e)$ and $X^{\pi}(v,e)$, we have
    \begin{align} \label{equ:XK}
\sum_{k=1}^m X_k(e) = \sum_{\pi \in \Pi} \sum_{v \in V} \text{deg}(v) \cdot X^{\pi}(v,e)
    \end{align}
    where $\text{deg}(v)$ is the degree of $v$ in $H$. 

    The following lemma (whose statement is similar to Lemma~3.5 in \cite{onak2012near}) is crucial for the analysis and we will prove it later.

    \begin{lemma}\label{lem:ot-3.5}
    For any edge $e$ and any $k \in [m-1]$, $X_{k+1}(e)-X_k(e) = O((m-2)!\cdot d_{\max})$
    \end{lemma}

    We first prove Lemma~\ref{lem:ot-main} given Lemma~\ref{lem:ot-3.5}.

    \begin{proof}[Proof of Lemma~\ref{lem:ot-main}]
    For any $\pi \in \Pi$, consider the edge $e = \pi_1$. When calling $VO^{\pi}(v_a(e))$ or $VO^{\pi}(v_b(e))$, the algorithm will only call $MO^{\pi}(e)$ and then terminate. So for any $\pi$ and $e$, $X^{\pi}(v_a(\pi_1),e)+X^{\pi}(v_b(\pi_1),e) = 2$ if $e = \pi_1$ and $0$ otherwise. This means 
    $$X_1(e) = \sum_{\pi_1 = e} 2 = 2(m-1)!$$.
    By Lemma~\ref{lem:ot-3.5}, for any $k$, 
    $$X_k(e) = 2(m-1)!+O(k \cdot (m-2)! \cdot d_{\max}) = O((m-1)! \cdot d_{\max})$$
    So for any edge $e$,
    $\sum_{k=1}^{m} X_k(e) = O(m!\cdot d_{\max})$. Together with Equation~(\ref{equ:XK}) and $\text{deg}(v) \ge d_{\min}$ for any $v \in V$, we have 
    $$
    \sum_{\pi \in \Pi} \sum_{v \in V} X^{\pi}(v,e)  = O\Paren{m! \cdot \frac{d_{\max}}{d_{\min}}}
    $$
    So
    \begin{align*}
\frac{1}{n} \cdot \frac{1}{m!} \cdot \sum_{\pi \in \Pi} \sum_{v \in V} N(\pi,v) 
    &= \frac{1}{n} \cdot \frac{1}{m!} \cdot \sum_{\pi \in \Pi} \sum_{v \in V} \sum_{e \in E} X^{\pi}(v,e) \\
       &= \frac{1}{n} \cdot \frac{1}{m!} \cdot \sum_{e \in E} O\Paren{m! \cdot \frac{d_{\max}}{d_{\min}}} \\
       &= \frac{m}{n} \cdot O\Paren{\frac{d_{\max}}{d_{\min}}} \\
       &=O\Paren{\frac{d_{\max}}{d_{\min}} \cdot \bar{d}}
       \end{align*}
       \end{proof}

       We now give the proof of Lemma~\ref{lem:ot-3.5}. 

       \begin{proof}[Proof of Lemma~\ref{lem:ot-3.5}]
       We first define some notation. For any $i \in \{0,1,2\}$, Let $\Pi_k^i$ be the set of permutations such that $\pi_k$ and $\pi_{k+1}$ have $i$ common endpoints. For any $\pi$, let $\pi'$ be the permutation such that $\pi'_k = \pi_{k+1}$, $\pi'_{k+1}=\pi_k$ and $\pi'_j = \pi_j$ for any $j$ not equal to $k$ or $k+1$. For any $i \in \{0,1,2\}$, $\pi \in \Pi_k^i$ if and only if $\pi' \in \Pi_k^i$. We have
       \begin{align*}
       & X_{k+1}(e) - X_k(e) \\
           = & \sum_{\pi \in \Pi} \Paren{X^{\pi}(v_a(\pi_{k+1}),e)+X^{\pi}(v_b(\pi_{k+1}),e)} - \sum_{\pi \in \Pi} \Paren{X^{\pi}(v_a(\pi_k),e)+X^{\pi}(v_b(\pi_k),e)} \\
           = &\sum_{i=1}^3 \Bracket{ \sum_{\pi \in \Pi_k^i} \Paren{X^{\pi}(v_a(\pi_{k+1}),e)+X^{\pi}(v_b(\pi_{k+1}),e)} - \sum_{\pi \in \Pi_k^i} \Paren{X^{\pi}(v_a(\pi_k),e)+X^{\pi}(v_b(\pi_k),e)} }\\
           \end{align*}
           For any $\pi \in \Pi^2_k$, $\pi_{k+1}$ and $\pi_k$ are parallel edges. So 
           $$
           \sum_{\pi \in \Pi_k^2} \Paren{X^{\pi}(v_a(\pi_{k+1}),e)+X^{\pi}(v_b(\pi_{k+1}),e)} - \sum_{\pi \in \Pi_k^2} \Paren{X^{\pi}(v_a(\pi_k),e)+X^{\pi}(v_b(\pi_k),e)} = 0
           $$
           For any $\pi \in \Pi^1_k$, $\pi_{k+1}$ and $\pi_k$ have only one common endpoint. So
           \begin{align*}
           & \sum_{\pi \in \Pi_k^1} \Paren{X^{\pi}(v_a(\pi_{k+1}),e)+X^{\pi}(v_b(\pi_{k+1}),e)} - \sum_{\pi \in \Pi_k^1} \Paren{X^{\pi}(v_a(\pi_k),e)+X^{\pi}(v_b(\pi_k),e)} \\
               = & \sum_{\pi \in \Pi_k^1} \Paren{X^{\pi}(v_a(\pi_{k+1}),e)+X^{\pi}(v_b(\pi_{k+1}),e) - X^{\pi}(v_a(\pi_k),e)-X^{\pi}(v_b(\pi_k),e)} \\
               = & \sum_{\pi \in \Pi_k^1} \Paren{X^{\pi}(v_c(\pi_{k+1},\pi_k),e)+X^{\pi}(v_d(\pi_{k+1},\pi_k),e) - X^{\pi}(v_c(\pi_k,\pi_{k+1}),e)-X^{\pi}(v_d(\pi_k,\pi_{k+1}),e)} \\
               = & \sum_{\pi \in \Pi_k^1} X^{\pi}(v_d(\pi_{k+1},\pi_k),e) - \sum_{\pi \in \Pi_k^1} X^{\pi}(v_d(\pi_{k},\pi_{k+1}),e) \\
               = & \sum_{\pi \in \Pi_k^1} X^{\pi}(v_d(\pi_{k+1},\pi_k),e) - \sum_{\pi \in \Pi_k^1} X^{\pi'}(v_d(\pi'_{k},\pi'_{k+1}),e) \\
               = & \sum_{\pi \in \Pi_k^1} \Paren{X^{\pi}(v_d(\pi_{k+1},\pi_k),e) - X^{\pi'}(v_d(\pi_{k+1},\pi_k),e)}
               \end{align*}
               For any $\pi \in \Pi^0_k$, $\pi_{k+1}$ and $\pi_k$ have no common endpoint. So
               \begin{align*}
               & \sum_{\pi \in \Pi_k^0} \Paren{X^{\pi}(v_a(\pi_{k+1}),e)+X^{\pi}(v_b(\pi_{k+1}),e)} - \sum_{\pi \in \Pi_k^0} \Paren{X^{\pi}(v_a(\pi_k),e)+X^{\pi}(v_b(\pi_k),e)} \\
                   =& \sum_{\pi \in \Pi_k^0} \Paren{X^{\pi}(v_a(\pi_{k+1}),e)+X^{\pi}(v_b(\pi_{k+1}),e)} - \sum_{\pi \in \Pi_k^0} \Paren{X^{\pi'}(v_a(\pi'_k),e)+X^{\pi'}(v_b(\pi_k),e)} \\
                   =& \sum_{\pi \in \Pi_k^0} \Paren{X^{\pi}(v_a(\pi_{k+1}),e) - X^{\pi'}(v_a(\pi_{k+1}),e)+X^{\pi}(v_b(\pi_{k+1}),e) - X^{\pi'}(v_b(\pi_{k+1}),e}
                           \end{align*}
                           For any $\pi$,$v$ and $e$, let $Y^{\pi}(v,e) = X^{\pi}(v,e) - X^{\pi'}(v,e)$, then
                           $$
                           X_{k+1}(e) - X_k(e) = \sum_{\pi \in \Pi_k^1} Y^{\pi}(v_d(\pi_{k+1},\pi_k),e) + \sum_{\pi \in \Pi_k^0} \Paren{Y^{\pi}(v_a(\pi_{k+1}),e) + Y^{\pi}(v_b(\pi_{k+1}),e)}
                           $$
                           We first prove the following lemma.
                           \begin{lemma} \label{lem:ot-Y}
                           For any $\pi$, $v$ and $e$, if $v$ is incident on $\pi_{k+1}$ but not incident on $\pi_k$, then $Y^{\pi}(v,e) = 1$ only if there is a sequence of calls to the matching oracle starting with
                           $\pi_{k+1}$, going on to $\pi_k$, and eventually leading to $e$.
                          The sequence also occurs when calling $MO^{\pi}(\pi_{k+1})$ directly.
                           \end{lemma}

                           \begin{proof}
                           Since $v$ is not incident on $\pi_{k}$, $VO^{\pi}(v)$ cannot directly call $MO^{\pi}(\pi_k)$. The only difference between a call to $VO^{\pi}(v)$ and $VO^{\pi'}(v)$ is that $MO^{\pi}(\pi_{k+1})$ may call $MO^{\pi}(\pi_k)$ but $MO^{\pi'}(\pi_{k+1})$ cannot call $MO^{\pi'}(\pi_k)$. So if $MO^{\pi}(e)$ is called when calling $VO^{\pi}(v)$ but not $VO^{\pi'}(v)$, it is called along the sequence starting with $MO^{\pi}(\pi_{k+1}),MO^{\pi}(\pi_k)$.

                           To prove the second part, notice that the only difference between calling $MO^{\pi}$ by $VO^{\pi}$ and calling $MO^{\pi}$ directly is that if it is called by $VO^{\pi}$, there are already several edges $e'$ such that $MO^{\pi}(e')$ has already been called. So there are more shortcuts in this case, which means any calling sequence that contains $MO^{\pi}(\pi_{k+1})$ and occurs in a call to $VO^{\pi}(v)$ also occurs in a call to $MO^{\pi}(\pi_{k+1})$.
                           \end{proof}

                           For any $e$, let $\Pi_e$ be the set of permutations such that $MO^{\pi}(e)$ occurs in a sequence of calls $MO^{\pi}(\pi_{k+1}),MO^{\pi}(\pi_k) \dots, MO^{\pi}(e)$ when calling $MO^{\pi}(\pi_{k+1})$ directly. For any $\pi \in \Pi_k^1$, $v_d(\pi_{k+1},\pi_k)$ is not incident on $\pi_k$, and for any $\pi \in \Pi_k^0$, both $v_a(\pi_{k+1})$ and $v_b(\pi_{k+1})$ are not incident on $\pi_k$. So by Lemma~\ref{lem:ot-Y}, we have
                           $$
                           X_{k+1}(e) - X_k(e) \le 2 \card{\Pi_e}
                           $$

                   For any $e'$ that conflicts with $e$, let $\Pi_{e,e'}$ be the set of permutations such that there is a sequence $MO^{\pi}(\pi_{k+1}), MO^{\pi}(\pi_k), \dots ,MO^{\pi}(e'),MO^{\pi}(e)$ that occurs in the call to $MO^{\pi}(\pi_{k+1})$. Let $\Pi_{e,e'}^1$ be the set of permutations of $\pi$ such that $\pi_{k+1}=e'$, $\pi_k=e$ and $\pi \in \Pi_{e,e'}$. Let $\Pi_{e,e'}^0$ be the set of permutations of $\pi$ such that $\pi_{k+1}=e'$, $\pi_k=e$ but $\pi \notin \Pi_{e,e'}$. Let $\Pi_{e,e'}^{\neg} = \Pi_{e,e'} \setminus \Pi_{e,e'}^1$. The following lemma is equivalent to Lemma~2.4 in \cite{yoshida2012improved}.

                   \begin{lemma} [Lemma~2.4 in \cite{yoshida2012improved}] \label{lem:ot-inj}
                   There is an injection from $\Pi_{e,e'}^{\neg}$ to $\Pi_{e,e'}^0$.
                   \end{lemma}

                   By Lemma~\ref{lem:ot-inj}, $\card{\Pi_{e,e'}} \le \card{\Pi_{e,e'}^0}+\card{\Pi_{e,e'}^1} = (m-2)!$. Since any edge $e$ only conflicts with at most $2d_{\max}-1$ edges, we have
                   $$
                   X_{k+1}(e)-X_k(e) \le 2 \card{\Pi_e} = 2 \sum_{e' \text{ conflicts with }e} \card{\Pi_{e,e'}} \le (4d_{\max}-2) (m-2)! = O\Paren{(m-2)! \cdot d_{\max}}
                   $$
                   This finishes the proof of Lemma~\ref{lem:ot-3.5}.
                   \end{proof} 
                   
                  \paragraph{Remark:} While not needed for our problem, the following stronger statement is a direct consequence of the proof.
                  
                  \begin{corollary}
                  If $H$ is a graph where in addition to conflicts between edges that share endpoints, each edge conflicts with at most $k$ other edges, and $\pi$ and $v$ are chosen randomly, then the vertex oracle, $VO^{\pi}$ makes at most
                  $O(\frac{(d_{\max} + k) \bar{d}}{d_{\min}})$ calls to $MO^{\pi}$ in expectation. Also $VO^{\pi}$ makes at most $\tilde{O}(\frac{(d_{\max} + k) \bar{d}}{d_{\min}})$ neighbor queries.
                  
                  
                  \end{corollary}




==> app_reduction.tex <==
\section{Omitted Details from Section~\ref{sec:tsp_vs_matchingsize}}
\label{sec:app-red}
\begin{lemma*} [Restatement of Lemma~\ref{lem:red-1}]
 Let $M$ be any matching in $G$. Then there is a $(1,2)$-TSP tour $T$ in $G'$ of cost at most $5n-\card{M}$.
\end{lemma*}

\begin{proof}
    Let $f: [n] \rightarrow [n]$ be any bijection from $[n]$ to $[n]$ such that whenever a vertex $v^1_i$ is matched to a vertex $v^2_j$ in $M$, then $f(i) = j$. Consider the following $(1,2)$-TSP tour $T$: each vertex $v^0_i \in V_0$ connects to $v^1_{2i-1}$ and $v^1_{2i}$ in $T$; each vertex $v^1_i \in V_1$ connects to $v^0_{\lceil (i+1)/2 \rceil}$ and $v^2_{f(i)}$ in $T$. For any $v^2_{f(i)} \in V_2$, it connects to $v^1_i$ and $v^3_{f(i)}$ in $T$. For any vertex $v^3_{f(i)} \in V_3$, if $i>1$, it connects to $v^2_{f(i)}$ and $v^4_{\ceil{i/2}}$ in $T$; if $i=1$, it connects to $v^2_{f(i)}$ and $v^4_{n/2}$ in $T$. See Figure~\ref{fig:reduction}(b) as an illustration. $T$ is clearly a TSP-tour. 
    
%  {\bf Sanjeev: It should be $i = 1$ above, right? Also, we need to argue that $T$ is connected.}

    All edges in $T$ are also edges in $G'$ except for possibly some edges between $V_1$ and $V_2$. If $v^1_i$ is matched in $M$, then $(v^1_i,v^2_{f(i)})$ is an edge in $G'$, otherwise it is not in $G'$ and thus has weight $2$. So $T$ only has $n-\card{M}$ weight $2$ edges, which means $T$ has cost at most $4n+n-\card{M}=5n-\card{M}$.
\end{proof}

\begin{lemma*} [Restatement of Lemma~\ref{lem:red-2}]
    For any $(1,2)$-TSP tour $T$ in $G$, $T$ has cost at least $5n-\alpha(G)$.
\end{lemma*}

We first prove an auxiliary claim.

\begin{claim} \label{cla:red}
    Suppose $G=(V_1,V_2,E)$ is a bipartite graph which has maximum size $\alpha(G)$. For any $2$-degree subgraph $H$ of $G$, if there are at most $X$ vertices in $V_1$ has degree $2$ in $H$, then there are at most $\alpha(G)+X$ vertices in $V_2$ which have degree at least $1$ in $H$. Similarly, if there are at most $X$ vertices in $V_2$ has degree $2$ in $H$, then there are at most $\alpha(G)+X$ vertices in $V_1$ which have degree at least $1$ in $H$.
\end{claim}

\begin{proof}
    If there are at most $X$ vertices in $V_1$ has degree $2$ in $H$. We construct $H'$ by deleting an arbitrary edge on each degree $2$ vertex in $V_1$, then construct $H''$ by deleing an arbitrary edge on each degree $2$ vertex in $V_2$. Since $H''$ does not have degree two vertex, it is a matching of $G$. So the number of degree $1$ vertices in $V_2$ in $H''$ is at most $\alpha(G)$. On the other hand, any vertex in $V_2$ which has degree at least $1$ in $H'$ also has degree $1$ in $H''$. So there are at most $\alpha(G)$ vertices of degree at least $1$ in $V_2$ in $H'$. Furthermore, since there are only $X$ vertices of degree $2$ in $V_1$ in $H$, we delete at most $X$ edges in $H$ when constructing $H'$. So $H'$ has at most $X$ more isolate vertices in $V_2$ than in $H$, which means $H$ has at most $\alpha(G)+X$ vertices with degree at least $1$ in $V_2$.

    The second part of the claim follows via a similar argument as the first part of the claim.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:red-2}]
    Let $a_{01}$ be the number of edges in $T \cap E_{0,1}$, $a_{2,3}$ be the number of edges in $T \cap E_{3,4}$. Let $G^X$ be the intersection graph of $G$ and $T$. Since the vertices in $V_0$ only connect to the vertices in $V_1$ in $G'$, and any vertex in $T$ has degree $2$, there are at least $n-a_{01}$ edges incident on $V_0$ in $T$ are not an edge in $G'$. On the other hand, since any vertex in $V_1$ is incident on at at most $1$ edge in $E_{0,1}$, there are at least $a_{01}$ vertices in $V_1$ is connected to a vertex in $V_0$ in $T$, which means there are at most $n-a_{01}$ vertices in $V_1$ has degree $2$ in $G^X$. By Claim~\ref{cla:red}, there are at most $n-a_{01}+\alpha(G)$ vertices in $V_2$ has edge in $G^X$. For any isolate vertex in $V_2$ in $T$, it has only one edge in $G'$ connecting to $V_3$, so this vertex must incident on an edge in $T$ which is not in $G'$. So there are at least $n-(n-a_{01}+\alpha(G)) = \alpha(G)-a_{01}$ edges incident on $V_2$ in $T$ which is not in $G'$.

    There are $2n$ edges incident on $V_3$ in $T$, but among them, there are only $a_{23}$ edges between $V_2$ and $V_3$ which is also in $G'$, and there are at most $n$ edges between $V_3$ and $V_4$ in $T$ since each vertex has degree only $2$. So there are at least $2n-n-a_{23}=n-a_{23}$ edges incident on $V_3$ which is not in $G'$. On the other hand, since any vertex in $V_2$ is incident on at at most $1$ edge in $E_{2,3}$, there are at least $a_{23}$ vertices in $V_2$ is connected to a vertex in $V_3$ in $T$, which means there are at most $n-a_{23}$ vertices in $V_2$ has degree $2$ in $G^X$. By Claim~\ref{cla:red}, there are at most $n-a_{23}+\alpha(G)$ vertices in $V_1$ has edge in $G^X$. For any isolate vertex in $V_1$ in $T$, it has only one edge in $G'$ connecting to $V_0$, so this vertex must incident on an edge in $T$ which is not in $G'$. So there are at least $n-(n-a_{23}+\alpha(G))=a_{23}-\alpha(G)$ edges incident on $V_1$ in $T$ which is not in $G'$.

    Since any edge has two endpoints, the number of edges in $T$ but not in $G'$ is at least $((n-a_{01})+(a_{01}-\alpha(G))+(n-a_{23})+(a_{23}-\alpha(G)))/2 = n-\alpha(G)$, which means $T$ has cost at least $4n+n-\alpha(G)=5n-\alpha(G)$.
\end{proof}


==> fig-mat-pair.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}
	\node[ellipse, black, fill=black!5, draw, line width=1pt, minimum width=100pt, minimum height=30pt] (S2) {$L(G_{S_2})$};
	\node[ellipse, black, fill=black!5, draw, line width=1pt, minimum width=100pt, minimum height=30pt] (S1) [above left = 40pt and 10pt of S2.center] {$L(G_{S_1})$};

	\node (A1) [left = 0pt of S2.center]{};
	\node (A2) [left = 10pt of A1]{};
	\node (A3) [left = 10pt of A2]{};

	\node (B1) [above = 50pt of A1]{};
	\node (B2) [above = 50pt of A2]{};
	\node (B3) [above = 50pt of A3]{};

	\draw (A1) to (B1);
	\draw (A2) to (B2);
	\draw (A3) to (B3);

	
	
\end{tikzpicture}

\caption{Illustration of $H_P$} \label{fig:mat-pair}

\end{figure}

==> fig-one-two.tex <==
\begin{figure}[h!]
    \centering
        \subcaptionbox{ A degree $3$ vertex $v_i$ in $G$.
    }[0.2 \textwidth]{ 
\begin{tikzpicture}[ auto ,node distance =1cm and 2cm , on grid , semithick , state/.style ={ circle ,top color =white , bottom color = white , draw, black , text=black}, every node/.style={inner sep=0,outer sep=0}]

\node[state, circle, black, line width=0.15mm, minimum height=20pt, minimum width=20pt] (a1) {$v_i$};
\node (b2) [right = 60pt of a1]{};
\node (b1) [above = 20pt of b2]{};
\node (b3) [below = 20pt of b2]{};

\draw (a1) to (b1) {};
\draw (a1) to (b2) {};
\draw (a1) to (b3) {};


                
\end{tikzpicture}
}
\hspace{2mm}  
        \subcaptionbox{ $v^1_i$ and $v^2_i$ in $G'$. 
    }[0.2 \textwidth]{  
\begin{tikzpicture}[ auto ,node distance =1cm and 2cm , on grid , semithick , state/.style ={ circle ,top color =white , bottom color = white , draw, black , text=black}, every node/.style={inner sep=0,outer sep=0}]

\node[state, circle, black, line width=0.15mm, minimum height=20pt, minimum width=20pt] (a1) {$v^1_i$};
\node (b2) [right = 60pt of a1]{};
\node (b1) [above = 20pt of b2]{};
\node (b3) [below = 20pt of b2]{};

\node[state, circle, black, line width=0.15mm, minimum height=20pt, minimum width=20pt] (a2) [above = 60pt of a1] {$v^2_i$};


\draw (a1) to (b1) {};
\draw (a1) to (b2) {};
\draw (a1) to (b3) {};
\draw [bend left] (a1) to (a2) {};
\draw [bend right] (a1) to (a2) {};
\draw [in = 40, out=-40, loop] (a2) to (a2) {};


\node[right = 53pt of a2] (t0) {};
\node[above = 5pt of t0] (t1) {\footnotesize $32n/\eps + 3$};
\node[below = 5pt of t0] (t2) {\footnotesize self loops};

\node[right = 20pt of a2] (t3) {$\dots$};

                
\end{tikzpicture}
}
\hspace{2mm}  
        \subcaptionbox{ $u^1_i$, $u^2_i$, $w^1_i$ and $w^2_i$ in $H'$.
    }[0.5 \textwidth]{  
\begin{tikzpicture}[ auto ,node distance =1cm and 2cm , on grid , semithick , state/.style ={ circle ,top color =white , bottom color = white , draw, black , text=black}, every node/.style={inner sep=0,outer sep=0}]

\node[state, circle, black, line width=0.15mm, minimum height=20pt, minimum width=20pt] (a1) {$w^1_i$};
\node (b2) [right = 60pt of a1]{};
\node (b1) [above = 20pt of b2]{};
\node (b3) [below = 20pt of b2]{};

\node[state, circle, black, line width=0.15mm, minimum height=20pt, minimum width=20pt] (a2) [above = 60pt of a1] {$w^2_i$};


\draw (a1) to (b1) {};
\draw (a1) to (b2) {};
\draw (a1) to (b3) {};
\draw [bend left] (a1) to (a2) {};
\draw [bend right] (a1) to (a2) {};

\node[state, circle, black, line width=0.15mm, minimum height=20pt, minimum width=20pt] (c1) [left = 80pt of a1] {$u^1_i$};
\node (d2) [left = 60pt of c1]{};
\node (d1) [above = 20pt of d2]{};
\node (d3) [below = 20pt of d2]{};



\node[state, circle, black, line width=0.15mm, minimum height=20pt, minimum width=20pt] (c2) [above = 60pt of c1] {$u^2_i$};


\draw (c1) to (d1) {};
\draw (c1) to (d2) {};
\draw (c1) to (d3) {};
\draw [bend left] (c1) to (c2) {};
\draw [bend right] (c1) to (c2) {};
\draw [bend left] (a2) to (c2) {};
\draw [bend right] (a2) to (c2) {};


\node[left = 40pt of a2] (t0) {$\dots$};
\node[above = 35pt of t0] (t1) {\footnotesize $32n/\eps + 3$};
\node[above = 25pt of t0] (t2) {\footnotesize parallel edges};

                
\end{tikzpicture}
}
    \caption{Construction of $G'$ and $H'$ focusing on a degree $3$ vertex in $G$. Here $n = 5$.}
    \label{fig:one-two}

\end{figure}



==> intro-reordered.tex <==
\section{Introduction}

In the metric traveling salesman problem (TSP), we are given $n$ points in an arbitrary metric space with an $n \times n$ matrix $D$ specifying pairwise distances between them. The goal is to find a simple cycle (a TSP tour) of minimum cost that visits all $n$ points. An equivalent view of the problem is that we are given a complete weighted undirected graph $G(V,E)$ where the weights satisfy triangle inequality, and the goal is to find a Hamiltonian cycle of minimum weight. The study of metric TSP is intimately connected to many algorithmic developments, and the poly-time approximability of metric TSP and its many natural variants are a subject of extensive ongoing research (see, for instance,~\cite{Vygen2012_Survey, sebo2014shorter, AnKS15, KarpinskiLS15, momke2016removing, SeboZ16, Gao18, TraubV18, MnichM18, TraubV19} and references within for some relatively recent developments). In this paper, we consider the following question: can one design sublinear algorithms that can be used to obtain good estimates of the cost of an optimal TSP tour? Since the complete description of the input metric is of size $\Theta(n^2)$, the phrase sublinear here refers to algorithms that run in $o(n^2)$ time. 

We first describe the results we prove in this paper and then provide the background and related work.

On the algorithmic side, we first consider the {\em graphic TSP} problem, an important case of metric TSP that has been extensively studied in the classical setting -- the metric $D$ corresponds to the shortest path distances in a connected unweighted undirected graph~\cite{momke2016removing,mucha2014frac,sebo2014shorter}. We give the first $\tilde{O}(n)$ time algorithm for graphic TSP that achieves an approximation factor better than 2.

\begin{theorem}
\label{thm:graphic_tsp_linear}
There is an $\tilde{O}(n)$ time randomized algorithm that estimates the cost of graphic TSP to within a factor of $2-\eps_0$ for some constant $\eps_0>0$.
\end{theorem}

On the other hand, if we are willing to allow a higher sublinear time, we can get a better approximation ratio.

\begin{theorem}
\label{thm:graphic_tsp_1.5}
There is an $\tilde{O}(n^{1.5})$ time randomized algorithm that estimates the cost of graphic TSP to within a factor of $(27/14)$. 
\end{theorem}

Our approach for estimating graphic TSP cost in sublinear time also lends itself to an $\tilde{O}(n)$ space streaming algorithm that can obtain an even better estimate of the cost. To our knowledge, no estimate better than a $2$-approximation was known previously. In the streaming model, we assume that the input to graphic TSP is presented as a sequence of edges of the underlying graph $G$. Any algorithm for this model, clearly also works if instead the entries of the distance matrix are presented in the stream -- an entry that is $1$ corresponds to an edge of $G$, and it can be ignored otherwise as a non-edge. 

\begin{theorem}
\label{thm:graphic_tsp_stream_main}
There is an $O(n)$ space randomized streaming algorithm that estimates the cost of graphic TSP to within a factor of $(11/6)$ in insertion-only streams. 
\end{theorem}


We next consider another well-studied special case of metric TSP, namely, $(1,2)$-TSP where all distances are either $1$ or $2$~\cite{adamaszek2018new,berman20068,papadimitriou1993traveling}, and obtain the following result.

\begin{theorem}
\label{thm:1,2_tsp_main}
There is an $\tilde{O}(n^{1.5})$ time randomized algorithm that estimates the cost of $(1,2)$-TSP  to within a factor of $1.625$. 
\end{theorem}

Note for both graphic TSP and $(1,2)$-TSP, we can trivially approximate the sizes of the TSP to within a factor 2 by simply outputting $2n$. In the $(1,2)$-TSP case this is immediately clear because any tour
must be of size between $n$ and $2n$. In the case of the graphic TSP, we know that the MST is of size $n-1$, and hence the TSP is of size between $n$ and $2n-2$.

It is easy to show that randomization is crucial to getting better than a $2$-approximation in sublinear time for both graphic TSP and $(1,2)$-TSP  -- see Theorem~\ref{thm:det_lower_bound} in Section~\ref{sec:det}. The algorithms underlying Theorems~\ref{thm:graphic_tsp_1.5} and~\ref{thm:1,2_tsp_main}, lend themselves to $\tilde{O}(n)$ space single-pass streaming algorithms with identical approximation guarantees. 
These sublinear time algorithms motivate the natural question if analogously to metric MST, there exist sublinear time algorithms that for any $\eps > 0$, output a $(1 + \eps)$-approximate estimate of TSP cost for graphic TSP and $(1,2)$-TSP in $\tilde{O}(n)$ time. We rule out this possibility in a strong sense for both graphic TSP and $(1,2)$-TSP.

\begin{theorem}
\label{thm:ptas_lowerbound_main}
There exists an $\eps_0 > 0$, such that any algorithm that estimates the cost of graphic TSP ($(1,2)$-TSP) to within a $(1 + \eps_0)$-factor, necessarily requires $\Omega(n^2)$ queries. 
\end{theorem}

Finally, similar to many classical approximation algorithms for TSP, our sublinear time estimation algorithms utilize subroutines for estimating the size of a maximum matching in the underlying graph. We show that this is not merely an artifact of our approach.

\begin{theorem}
\label{thm:tsp_vs_matchingsize_main}
For any $\eps \in [0,1/5)$, any algorithm that estimates the cost of an $n$-vertex instance of graphic TSP or $(1,2)$-TSP to within a $(1 + \eps)$-factor, can also be used to estimate the size of a maximum matching in an $n$-vertex bipartite graph to within an $\eps n$ additive error, with an identical query complexity, running time, and space usage.
\end{theorem} 

This connection allows us to translate known lower bounds for matching size estimation in various models to similar lower bounds for metric TSP cost estimation. In particular, using the results of~\cite{assadi2017estimating}, we can show that there exists an $\eps_0$ such that any randomized single-pass dynamic streaming algorithm for either graphic TSP or $(1,2)$-TSP that estimates the cost to within a factor of $(1+\eps_0)$, necessarily requires $\Omega(n^2)$ space. 


We now provide further elaboration of these results and the preceding work on which they are based.


A standard approach to estimating the metric TSP cost is to compute the cost of a minimum spanning tree, and output two times this cost as the estimate of the TSP cost (since any spanning tree can be used to create a spanning simple cycle by at most doubling the cost). 
The problem of approximating the cost of the minimum
spanning tree in sublinear time was first studied in the graph adjacency-list model by Chazelle, Rubinfeld, and Trevisan~\cite{ChazelleRT05}. The authors gave an $\tilde{O}(d W /\eps^2)$-time algorithm to estimate the MST cost to within a $(1+\eps)$-factor in a graph where average degree is $d$, and all edge costs are integers in $[1..W]$. For certain parameter regimes this gives a sublinear time algorithm for estimating the MST cost but in general, this run-time need not be sublinear.
Subsequently, in an identical setting as ours, Czumaj and Sohler~\cite{czumaj2009estimating} showed that for any $\eps > 0$, there exists an $\tilde{O}(n/\eps^{O(1)})$ time algorithm that returns a $(1 + \eps)$-approximate estimate of the MST cost when the input is an $n$-point metric. This result immediately implies an $\tilde{O}(n/\eps^{O(1)})$ time algorithm to estimate the TSP cost to within a $(2 + \eps)$ factor for any $\eps > 0$. However, no $o(n^2)$ query algorithms are known to approximate metric TSP to a factor that is strictly better than $2$. On the other hand, there are also no known barriers that rule out existence of $(1 + \eps)$-approximate estimation algorithms for metric TSP with $\tilde{O}(n)$ queries for any fixed $\eps > 0$. In this paper, we make progress on both algorithms and lower bounds for estimating metric TSP cost.


At a high-level, our algorithm is based on showing the following: if a graph $G$ either lacks a matching of size $\Omega(n)$ or has $\Omega(n)$ biconnected components (blocks), then the optimal TSP cost is not too much better than $2n$. Conversely, if the graph $G$ has both a large matching and not too many blocks, then we can show that the optimal TSP cost is distinctly better than $2n$. Since we do not know an efficient sublinear algorithm to estimate the number of blocks in a graph $G$, we work with another quantity that serves as a proxy for this and can be estimated in $\tilde{O}(n)$ time. The main remaining algorithmic challenge then is to estimate sufficiently well the size of a largest matching. This problem is very important by itself, and has received much attention~\cite{PR07,NguyenO08,yoshida2012improved,onak2012near,kapralov2020space}; please see a detailed discussion of this problem, and relevant recent developments towards the end of this section. Our $\tilde{O}(n)$ query results utilize the recent result of Kapralov {\em et al.} \cite{kapralov2020space} who give an algorithm to approximate the size of maximum matching to within a constant factor (for some very large constant) in $\tilde{O}(n)$ time in the {\em pair query} model (is there an edge between a given pair of vertices?). We also show that matching size can be estimated to within a factor of $2$ in $\tilde{O}(n^{1.5})$ time (see proof of Theorem~\ref{lem:max-mat} in Section~\ref{sec:app-mat}), crucial to obtaining the approximation guarantee in Theorem~\ref{thm:graphic_tsp_1.5}. 


Throughout the paper, whenever we refer to a graph associated with a $(1,2)$-TSP instance, it refers to the graph $G$ induced by edges of distance $1$ in our $\{1,2\}$-metric. At a high-level, the idea underlying our algorithm is to analyze the structure of the graph $G$ induced by edges of distance $1$. 
We design an algorithm to estimate the size of a maximal ``matching pair'' of $G$ which is defined to be a pair of edge-disjoint matchings. We show that whenever the size of a matching pair is large in a graph $G$, the TSP cost is distinctly smaller than $2n$, and conversely, if this quantity is not large, the TSP cost is close to $2n$. The main remaining algorithm challenge then is to estimate sufficiently well the size of a maximal matching pair, and we show that this can be done in $\tilde{O}(n^{1.5})$ time (see proof of Theorem~\ref{lem:mat-pair} in Section~\ref{sec:mat-pair}). 

For $(1,2)$-TSP, an $\tilde{O}(n)$ query algorithm that estimates the cost of $(1,2)$-TSP to within a factor of $1.75$ was claimed in~\cite{sublinear71} but this result is based on the matching size estimation results of~\cite{onak2012near}. Unfortunately, as confirmed by the authors~\cite{onakpersonalcommunication}, there is a problem with the proof of one of the statements in the paper --- Observation 3.9 --- which is crucial for the correctness of the main result. 
As a result, the $\tilde{O}(d)$ time result in the neighbor query model as well as the $\tilde{O}(n)$ time result in the adjacency matrix, claimed in~\cite{onak2012near} can no longer be relied upon, and we have chosen to make this paper independent of these results~\cite{onak2012near}. It is worth mentioning that if the $\tilde{O}(n)$-time matching estimation result of~\cite{onak2012near} can be shown to hold, then the run-time of both Theorems~\ref{thm:graphic_tsp_1.5} and~\ref{thm:1,2_tsp_main} can be improved to $\tilde{O}(n)$ time.


This lower bound result highlights a sharp separation between the behavior of metric MST and metric TSP problems. At a high-level, our lower bound is inspired by the work of Bogdanov {\em et al.} \cite{bogdanov2002lower} who showed that any query algorithm that for any $\eps > 0$ distinguishes between instances of parity equations (mod $2$) that are either satisfiable (Yes) or at most $(1/2 + \eps)$-satisfiable (No), requires $\Omega(n)$ queries where $n$ denotes the number of variables. However, the query model analyzed in~\cite{bogdanov2002lower} is different from ours. The model in~\cite{bogdanov2002lower} allows queries of the form -- return the $j_{th}$ equation in which a given variable $x$ appears; in contrast, the query model suitable for our application requires understanding a weaker class of queries, namely, the algorithm can only ask queries of the form: does literal $\ell$ appear in equation $i$? We first show that the lower bounds of~\cite{bogdanov2002lower} can be shown to be $\Omega(n^2)$ for this weaker class. We then show that Yes and No instances of parity equations can be converted into instances of graphic TSP (resp. $(1,2)$-TSP) such that for some $\eps_0 > 0$, any $(1 + \eps_0)$-approximation algorithm for graphic TSP (resp. $(1,2)$-TSP), can distinguish between the Yes and No instances of the parity equations, giving us the desired result.


We conclude by establishing several additional lower bound results that further clarify the query complexity of approximating TSP cost. For instance, we show that if an algorithm can access an instance of graphic TSP by only querying the edges of the graph (via neighbor and pair queries), then any algorithm that approximates the graphic TSP cost to a factor better than $2$, necessarily requires $\Omega(n^2)$ queries (see Theorem~\ref{thm:graphic_tsp_lowerbound_standard_model}). This is in sharp contrast to Theorem~\ref{thm:graphic_tsp_linear}, and shows that working with the distance matrix is crucial to obtaining sublinear time algorithms for graphic TSP. We also show that even in the distance matrix representation, the task of {\em finding a  tour} that is $(2-\eps)$-approximate for any $\eps > 0$, requires $\Omega(n^2)$ queries for both graphic TSP and $(1,2)$-TSP (see Theorem~\ref{thm:solution}).

\smallskip
\noindent
{\bf Matching Size Estimation:}
As the problem of matching size estimation is intimately connected to metric TSP cost estimation, we briefly review some relevant work here. This line of research primarily assumes that we are given a graph $G(V,E)$ with maximum degree $d$, that can be accessed via 
{\em neighbor queries}~\cite{GoldreichR02}: (a) for any vertex $v$, we can query its degree, and (b) for any vertex $v$ and an integer $i$, we can learn the $i_{th}$ neighbor of $v$. 

Parnas and Ron~\cite{PR07} initiated the study of matching size estimation in sublinear time and gave an $d^{O(\log(d/\eps)}$ time algorithm that estimates the matching size to within a constant factor plus an additive $\eps n$ error for any $\eps > 0$. Nguyen and Onak~\cite{NguyenO08} presented a new estimation algorithm and showed that it can estimate the matching size to within a factor of $2$ plus an additive $\eps n$ error in $2^{O(d)}/\eps^2$ time. We will refer to this approximation guarantee as a {\em $(2,\eps)$-approximation} of matching size. Yoshida {\em et al.}~\cite{yoshida2012improved} strongly improved upon the performance guarantee obtained in~\cite{NguyenO08}, and showed that a $(2,\eps)$-approximation to matching size can be accomplished in $O(d^4/\eps^2)$ time (in fact, they obtain the stronger $(2 \pm \eps)$-approximation guarantee). 
The analysis of~\cite{yoshida2012improved} was further improved by Onak {\em et al.}~\cite{onak2012near} who showed that the state of the art for $(2,\eps)$-approximation of matching size. 
We note that it is known that any $(O(1),\eps)$-approximate estimate of matching size necessarily requires $\Omega(d)$ queries~\cite{PR07}, so the result of~\cite{onak2012near} is essentially best possible. Unfortunately, as mentioned above, we recently discovered a subtle mistake in the analysis of Onak {\em et al.}~\cite{onakpersonalcommunication}. Consequently, the best known time complexity for obtaining a $(2,\eps)$-approximate estimate is $\tilde{O}(d^2/\eps^2))$; this weaker result also follows from the work of ~\cite{onak2012near}, but does not rely on the incorrect observation in~\cite{onak2012near}.

The difference between a linear dependence versus a quadratic dependence on degree $d$ is however huge in the sublinear time applications when the graph is not very sparse. In particular, while an $\tilde{O}(d)$ query result translates into an $\tilde{O}(n)$ time algorithm in the adjacency matrix model, an $\tilde{O}(d^2)$ query result gives only an $\tilde{O}(n^2)$ time algorithm, which is clearly not useful. Very recently, Kapralov {\em et al.}~\cite{kapralov2020space} gave an alternate approach based on a vertex ``peeling'' strategy (originally proposed in~\cite{PR07}) that yields an $(O(1),\eps)$-approximation of matching size in $\tilde{O}(d/\eps^2)$ time. Unfortunately, the constant hidden in the $O(1)$ notation is very large, and efficiently obtaining a $(2,\eps)$-approximation to matching size remains an important open problem. Meanwhile, by directly building on the work of~\cite{yoshida2012improved}, we obtain an $\tilde{O}(n^{1.5})$ time algorithm for a $(2,\eps)$-approximation to matching size in the adjacency matrix model, and it is this algorithm that is used in the results of Theorem~\ref{thm:graphic_tsp_1.5} and Theorem~\ref{thm:1,2_tsp_main}. 

%%%It is worth highlighting if an alternate proof of the results in~\cite{onak2012near} is discovered, then the query and %%%time complexity of our algorithms in Theorem~\ref{thm:graphic_tsp_1.5} and Theorem~\ref{thm:1,2_tsp_main} will %%%immediately improve to $\tilde{O}(n)$.


\iffalse
%Onak {\em et al.}~\cite{onak2012near} consider the problem of computing a $(2,\eps)$-approximation to the size of the minimum vertex cover. Their algorithm works by estimating the size of a maximal matching in the graph.
 Yoshida {\em et al.}~\cite{yoshida2012improved}  consider the problem of estimating the size of a maximum matching, maximal independent set, and other related problems. The focus of \cite{yoshida2012improved} was on 
estimating these quantities in sparse graphs using a neighbor query model, where each query consists of a vertex $v$ and an integer $i$, and the answer is the $i^{th}$ neighbor of $v$. Yoshida {\em et al.}~\cite{yoshida2012improved} treat the average degree as a constant and do not optimize the dependence of their algorithm's performance on the average degree.
Onak {\em et al.}~\cite{onak2012near} seek to extend these results to dense graphs with a query model that is close to the one used in this paper, where each query is a pair of vertices and the answer is the entry in the appropriate adjacency matrix. In this model, they claimed an $\tilde{O} (n) \textrm{poly}(1/\eps )$-time algorithm for estimating the size of a maximal matching to within an $\eps n$ additive error. However, as mentioned earlier, this result is no longer known to be correct. Consequently, we build directly on the work of~\cite{yoshida2012improved}  in Theorem~\ref{thm:graphic_tsp_1.5} and Theorem~\ref{thm:1,2_tsp_main}. It is worth highlighting if an alternate proof of the results in~\cite{onak2012near} is discovered, then the query and time complexity of our algorithms in Theorem~\ref{thm:graphic_tsp_1.5} and Theorem~\ref{thm:1,2_tsp_main} will immediately improve to $\tilde{O}(n)$.
\fi


\smallskip
\noindent
{\bf Other Related Work:}
We note here that there is an orthogonal line of research that focuses on computing an approximate solution in near-linear time when the input is presented as a weighted undirected graph, and the metric is defined by shortest path distances on this weighted graph. It is known that in this model, for any $\eps > 0$, there is an $\tilde{O}(m/\eps^2 + n^{1.5}/\eps^3)$ time algorithm that computes a $(3/2 + \eps)$-approximate solution; here $n$ denotes the number of vertices and $m$ denotes the number of edges~\cite{CQ18}, and that a
$(3/2 + \eps)$-approximate estimate of the solution cost can be computed in $\tilde{O}(m/\eps^2 )$ time~\cite{CQ17}. It is not difficult to show that in this access model, even when the input graph is unweighted (i.e. a graphic TSP instance), any algorithm that outputs better than a $2$-approximate estimate of the TSP cost, requires $\Omega(n + m)$ time even when $m = \Omega(n^2)$. Hence this access model does not admit sublinear time algorithms that beat the trivial $2$-approximate estimate.

 \smallskip
 \noindent
 {\bf Organization:} In Section~\ref{sec:graph_TSP}, we present our algorithms for graphic TSP (Theorem~\ref{thm:graphic_tsp_linear} and Theorem~\ref{thm:graphic_tsp_1.5}). In section~\ref{sec:1,2_TSP}, we present the $1.625$-approximation algorithm of $(1,2)$-TSP (Theorem~\ref{thm:1,2_tsp_main}). In Section~\ref{sec:ptas_lower_bound}, we present our lower bound result that rules out possibility of a sublinear-time approximation scheme for both graphic TSP and $(1,2)$-TSP (Theorem~\ref{thm:ptas_lowerbound_main}). In Section~\ref{sec:tsp_vs_matchingsize}, we present a strong connection between approximating metric TSP cost and estimating matching size (Theorem~\ref{thm:tsp_vs_matchingsize_main}). Finally, in Appendix~\ref{sec:additional_lower_bounds}, we present several additional lower bound results on the complexity of approximating graphic TSP and $(1,2)$-TSP cost.  

